Better Data Labelling with EMBLEM (and how that Impacts Defect Prediction)

Standard automatic methods for recognizing problematic development commits can be greatly improved via the incremental application of human+artificial expertise. In this approach, called EMBLEM, an AI tool first explore the software development process to label commits that are most problematic. Humans then apply their expertise to check those labels (perhaps resulting in the AI updating the support vectors within their SVM learner). We recommend this human+AI partnership, for several reasons. When a new domain is encountered, EMBLEM can learn better ways to label which comments refer to real problems. Also, in studies with 9 open source software projects, labelling via EMBLEM's incremental application of human+AI is at least an order of magnitude cheaper than existing methods ($\approx$ eight times). Further, EMBLEM is very effective. For the data sets explored here, EMBLEM better labelling methods significantly improved $P_{opt}20$ and G-scores performance in nearly all the projects studied here.

==> fft.tex <==
Psychological scientists have developed FFTs (Fast and Frugal Trees) as one way
  to generate comprehensible models consisting of
   separate tiny rules~\cite{phillips2017fftrees,chen2018applications,martignon2008categorization}.
      A FFT is a decision tree made for binary classification problem with exactly two branches extending
        from each node, where either one or both branches is an exit
        branch leading to a leaf~\cite{martignon2008categorization}. 
        That is to say, in an FFT,  every question posed by a node will
        trigger an immediate decision
        (so humans can read every leaf node
        as a separate rule).



We used the similar implementation of FFT as offered by Fu and Chen et al.~\cite{fu2018building,chen2018applications}. 
An FFT of depth $d$ has a choice of two ``exit policies'' at each level: the existing branch can select for the negation of the target, i.e., non-severe, (denoted ``0'') or the target (denoted ``1''), i.e., severe.
The right-hand-side tree in Figure~\ref{fig:fft1} is 01110 since:
\bi
\item
The first level found a rule that exits to the negation of the target: hence, ``0''.
\item
While the next tree levels found rules that
exit first to target; hence, ``111''.
\item
And the final line of the model exits
to the opposite of the penultimate line; hence, the final ``0''.
\ei

\begin{figure}[!b]

 {\normalsize
\begin{minipage}{\linewidth}
\begin{tabular}{p{\linewidth}}
  \qquad  if  \qquad \ \ topic 1 $>$  0.80   \qquad \qquad  then false \qquad \#0 \\
  \qquad  else if \ \ topic 7 $>$  0.60    \qquad \qquad   then true \qquad \  \#1 \\
   \qquad else if \ \ topic 3 $>$  0.65   \qquad \qquad  then true \qquad \  \#1 \\
   \qquad else if \ \ topic 5 $\leq$ 0.50    \qquad \qquad  then true \qquad \  \#1 \\
   \qquad else \qquad \qquad \qquad \qquad \qquad \qquad false \qquad \qquad \ \#0 
\end{tabular}
\end{minipage}
}
\vspace{-0.25cm}
\caption{Example of an FFT}
\label{fig:fft1}
\end{figure}

Following the advice of~\cite{fu2018building,chen2018applications,phillips2017fftrees}, for all the experiments of this paper, we use a depth    $d=4$. 
For trees of depth $d=4$, there are $2^4=16$ possible trees which can be denoted as 00001, 00010, 00101, ... , 11110. During FFT training, all $2^d$ trees are generated, then we select the best one (using the training data).
 This single best tree is then applied to the test data.
 Note that FFTs of such small
depths are very succinct
(see examples in Figures~\ref{fig:fft} and~\ref{fig:fft1}). Such FFTs generate rules which leads to decision of finding a report as severe and non-severe for the datasets under study. Many other data mining algorithms used in software analytics are far less
succinct and far less comprehensible as explained in \tion{comprehensibility}.


% \begin{table}[!t]
% \caption{Comprehension issues with models generated by data mining algorithms used in software analytics.}\label{tab:bad}
% \begin{tabular}{|p{.99\linewidth}|}\hline
% \rowcolor{gray!20}
% For very high dimensional data, there is some evidence that complex deep learning algorithms
%     have  advantages for software engineering applications~\cite{yang2015deep, white2015toward,gu2016deep}. 
%     However, since they do not readily support   explainability, they have been  criticizing   as 
%     ``data mining alchemy''~\cite{DL2017alchemy}. \\

% Support vector machines and principle component methods achieve their results after synthesizing new dimensions
% which are totally unfamiliar to human users~\cite{Menzies2009ExplanationVP}.\\\rowcolor{gray!20}

% Other methods that are heavily based on mathematics can be hard to explain to most
% users. For example, in our experience, it is hard for (e.g.,) users to determine minimal changes to a project that mostly affect defect-proneness, just by browsing the internal frequency tables of a Naive Bayes classifier or the coefficients found via linear regression/logistic regression~\cite{Menzies2009ExplanationVP}.\\

% When decision tree learners  are many pages long, they are  hard to browse and understand~\cite{friedl1997decision}.\\\rowcolor{gray!20}

% Random forests are even harder to understand than decision trees since the problems of reading one tree are multiplied $N$ times, one for each member of the forest~\cite{liaw2002classification}. \\

% Instance-based methods do not compress their training data; instead they produce  conclusions by  finding older exemplars closest to the new example. Hence, for such instance-based methods, it is hard to generalize and make a conclusion about what kind of future projects might be (e.g.,) most defective-prone~\cite{aha1991instance}.
% \\\hline
% \end{tabular}
% \end{table}  


%  The value of models such as FFTs comprising many small rules has been extensively studied:
%  \bi
%  \item
%              These    models use very few
%              attributes from the data. Hence they tend to be robust against overfitting, especially on small and noisy data, and have been found to predict data at levels comparable with regression. See for example~\cite{martignon2008categorization, woike2017integrating,czerlinski1999good}.
%         \item
%         Other   work has  shown that these rule-based
%         models can perform comparably well to more  complex models in a range of domains
%         e.g., public health, medical risk management, performance science, etc.~\cite{jenny2013simple, laskey2014comparing, raab2015power}.
%         \item
%           Neth and Gigerenzer
%           argue that such rule-bases  are tools that   work well under conditions of uncertainty~\cite{neth2015heuristics}. 
%           \item
%       Brighton showed that rule-based models can perform better than 
%         complex nonlinear algorithms such as  neural networks, 
%         exemplar models, and classification/regression trees~\cite{brighton2006robust}.
%  \ei      

==> keywords.tex <==

\begin{table}
\caption{Keywords used to classify commit messages as corrective, adaptive,  or perfective issues.}\label{tab:words}
\scriptsize
\vspace{-10pt}
\begin{tabular}{|p{.95\linewidth}|}\hline
Corrective: active, against, already, bad, block, bug, build, call,case, catch, cause, character, compile, correctly, create, different,dump, error, except, exist, explicitly, fail, failure, fast, fix, format, good, hack, hard, help, init, instead, introduce, issue, lock, log,logic, look, merge, miss, null, oops, operation, operations,pass, previous, previously, probably, problem, properly, random,recent, request, reset, review, run, safe, set, similar, simplify, special, test, think, try, turn, valid, wait, warn, warning, wrong 
\vspace{0.1cm}

Adaptive: active, add, additional, against, already, appropriate, available, bad, behavior, block, build, call, case, catch,change, character, compatibility, compile, config, configuration, context, correctly, create, currently, default, differ-ent, documentation, dump, easier, except, exist, explicitly, fail,fast, feature, format, future, good, hack, hard, header, help,include, information, init, inline, install, instead, internal, introduce, issue, lock, log, logic, look, merge, method, necessary,new , old, operation, operations, pass, patch, previous, previously, probably, properly, protocol provide, random, recent, release, replace, request, require, reset, review, run, safe, security, set, similar, simple, simplify, special, structure, switch, test, text, think, trunk, try, turn, useful, user, valid, version, wait 
\vspace{0.1cm}

Perfective: cleanup, consistent, declaration, definition,header, include, inline, move, prototype, removal, static,style, unused, variable, warning, whitespace 
\\\hline
\end{tabular}
\vspace{-10pt}
\end{table}


==> lit_figure.tex <==
\pdfoutput=1
%\begin{figure}[ht]
\begin{figure}[t]
\vspace{-0.3cm}
%vspace{-32pt}
\begin{center}
    \includegraphics[width=0.47\textwidth]{lit_review.png}
\end{center}
\vspace{-0.2cm}
\caption{Literature review of hyperparameters tuning on 52 top defect prediction papers \cite{Fu16Grid}}\label{fig:litfigure}
\vspace{-0.5cm}
\end{figure}


==> old/reviewers_comments.tex <==
\clearpage
\appendix


\setcounter{page}{1}
\pagenumbering{roman}
\normalsize
\section*{Response to Reviewers}


{\em All reviewers raised   concerns regarding to the presentation, contribution, and evaluation of this paper. Addressing these concerns sufficiently would require a major revision.}


Thank you for allowing us to offer a revised version of the previous draft.
In the body of the paper,  the \revised{WORDS IN BLUE} shows exactly where we have updated this text.


Also, please note that 
as our draft went through major revision, we have disambiguate our terminology.
Our new contribution is now called
  ``EMBLEM'', which refers to labelling technology.

 
 
 
{\em   The vocabulary and terminology used are confusing from time to time.}

We have  addressed that problem in this draft.

{\em The reviewers also raised questions about the significance of the contribution, e.g. in modern projects, linking commits with issues has become common practice. }

You raised a good point - the last draft of this paper did not stress the main message  prominently enough. In this draft, please see: 

\bi
\item
The notes
on {\bf RQ3} on page1,2: there we show one example were a task costing \$320K and 39,000 hours (without our tools) would cost \$40K and 4,940 hours (with our tools).
\item
We have a most new Section~2 that offers much mroe detail
on why this paper is needed:
\bi
\item
Section 2.1 discusses the general
problem of how to do faster science. 
\item
Section 2.2 clearly distinguishes our labeling work from the other parts of the data mining pipeline.
\item
Also, 
please see the discussion around \tbl{gittracking}: mapping code fixing commits to their associated comments (and vice versa) is often done very poorly. \item
\tbl{gittracking} shows an example of that (and we note that other authors have raised similar concerns~\cite{herzig13_misclassifications, bird09_bias, Wu11_relink})
\ei
\ei
{\em The approach needs to be better explained and the evaluation should use state-of-the-art work as the baseline.
We look forward to receiving your revised manuscript.}

Please see the discussion around \tbl{gittracking}: mapping code fixing commits to their associated comments (and vice versa) is often done very poorly. \tbl{gittracking} shows an example of that (and we note that other authors have raised similar concerns~\cite{herzig13_misclassifications, bird09_bias, Wu11_relink})



 

\subsection*{Response to Reviewer \#1}

Please see the \revised{WORDS IN BLUE}, showing exactly where we have updated this draft.
Also, please see below for our responses to your specific comments.

One comment we make at the start: some of your remarks asked whether we focused
on labelling and not, e.g. better use of the SZZ algorithm (see R1-k later in this response). 
In reply, as shown on page 3 of the paper, we say that software analytics has many parts and no one paper can make contributions to all those parts.
The diagram on page3 shows nine parts of this pipeline. As we say in the text,
this paper is about part4 (Data labelling)
while SZZ methods are about part2 (data collection). Yes, indeed, perhaps even better results could be obtained by {\em combining} better labelling with better SZZ methods, but before anyone tries that, such future work would need
to be motivated by some initial results documenting the benefits of labelling. Hence, this paper.

\review{\textbf{R1-a:} This paper proposed to exploit two new techniques (i.e., EMBLEM and FAST FRUGAL TREES) to facilitate the task of commit labeling and just-in-time defect prediction respectively. The central insight of this paper is that the commit labeling problem is analogous to reading research papers. With an such intuition, the authors proposed to leverage an active learning approach, EMBLEM, to label “worrying” commits. The evaluation over 9 open source projects demonstrated the benefits of using the proposed ``F3T'' technique. \\
Defect prediction has attracted huge research attention a decade ago. Although it gets less and less attention recently, many research efforts are still being made to advance this direction. Labeling commits, on the other hand, seems to be more important since it is the foundation of many mining-based software engineering researches. Therefore, the motivation of this work, as emphasized in Section 2.3, is clear to me. \\
However, many enhancements could be made to improve this manuscript. Especially for its approach (i.e., not clearly explained) and evaluations (i.e., missing important state-of-the-art techniques). \\
1. The approach, including its intuition and insights, is too brief and confusing.} 

We appreciate your summary and as you have suggested, we have revised the paper's introduction and background sections more extensively. (See page 1-5) \\


\review{\textbf{R1-b:} The authors spent much  efforts in describing motivations and different learning models. However, the description of the approach itself is too brief, which prevent me from understanding the novelty of this work clearly. For instance, the central insight of this paper is “Commit labeling problem is analogous to reading research papers”.  However, there is no justification or examples why this insight might be valid. This poses significant threats to the validity of the proposed approach.} 

To address this point, we have given justification as both problem working towards identifying the relevant examples with least amount of inspection efforts by reading/labeling. \citeresp{1b} 

\review{\textbf{R1-c:} Besides, what is the intuition of use “FAST and FRUGAL TREES” in classifying buggy commits? Since it is a major component of the F3T approach, justifications are required.}

As for why we selected FFTs   that study was reported at FSE'18 \cite{di18_fft} where FFTs were shown to out-perform a wide sample of other methods, commonly used for defect prediction.


But, as you rightly pointed out,  the previous description of this work confused the core message with
some of the less-important implementation details.

Accordingly, we now focus here on our main message (the labeling) rather than certain less-important details (the learning method). We say FFTs are less important since, since in \tbl{rq2aaa}, we  compare the effects of using or not using FFTs in conjunction with the usage EMBLEM. The result there is very clear, if we use FFTs with EMBLEM, that wins over just using FFTs 
(without EMBLEM) in  7/9 cases 
(for both $P_{opt}20$ and G-score). Therefore, we say that the real message of this paper is EMBLEM and not FFTs.  

\review{\textbf{R1-d:} If we only look at the commit log messages, they are only text tokens. In such case, the approach EMBLEM can process the data of log messages if it can process research papers. However, the characteristics of log messages and research papers diverge a lot. Will that affect the effectiveness of EMBLEM in labeling commits?}

You are quite correct. Prior to this paper is was not known if a EMBLEM-style of analysis would fail since the  text data that EMBLEM explored was so different from the commit logs explored here. In fact, given that they were so different, our pre-experimental intuition exactly like yours;
i.e. this method {\em would} fail miserably.

Now the surprising result presented here is that those text differences {\bf did not} preclude
the use of that kind of analysis to this kind of textual data. 

Given the large differences in the text types, and the success of this analysis on both kinds of text, we now conjecture that ``reading'' (and, in particular, our kind of active reading)
could be applied to a wide variety of SE artifacts. Of course, that is just a speculation, drawing from our experiments, which would require further extensive analysis. But it is a promising direction for future work.

 
%You are quite correct and the concern regarding the effectiveness of EMBLEM in labeling commits is valid. However, our goal is to investigating if using EMBLEM can solve the labeling problem when comparing to existing methods and practically, it is still effective when being used to label commit logs that does improve the ``accuracy'' of the labels as ground truths (1) inspected by human and (2) defect prediction task. Further tuning and analysis can be done as future extension of this work. 

\review{\textbf{R1-e:} Besides, details of EMBLEM are also not clearly explained. In the description of Section 3, it seems that EMBLEM integrates some sampling techniques and machine learner (e.g., SVM) together. However, what are the features used here for the learner SVM? If EMBLEM requires generating a set of features to label commit, then what are the features generated for research papers in the original setting of EMBLEM?}

We have updated the draft with more details regarding EMBLEM framework. The features are the same as in the original setting suggested by Yu et al. \cite{Yu2018,Yu2019} with L2-normed 4000 top terms with highest tf-idf scores. \citeresp{1e}

\review{\textbf{R1-f:} In page 4 at line 41, ``until N2=30 relevant examples are found''. Here, are these 30 examples declared by human or automatically?}

Here, these 30 examples are declared by human.

\review{\textbf{R1-g:} Many notations in Table 3 have not been explained. It is not a good practice to present a table without explaining the items listed in it. The current description of Section 3 confused me in many aspects. I suggest the authors to enhance the explanation why EMBLEM can be applied in labeling commit, and use a diagram to better explain the workflow of EMBLEM.}

Thank you for this point, we have updated both Table 3 and Section 3 to address the issue as how EMBLEM can be applied in labeling commits with steps of the workflow included. \citeresp{1g}

\review{\textbf{R1-h:} 2. Some details are not well-explained. In RQ2, RQ3 and RQ4, the authors should discuss more details about whether the evaluation results on the manually labeled four projects are different from those on the other five automated labeled projects. The authors claimed that using FASTREAD, humans only need to read a small percentage of the commits (Page 4). However, the authors did not present the exact data that how many commits have been manually reviewed for each project. I think such information should be listed in the experimental setup.}

Thanks for pointing that out. The evaluation process is different both the first four manually labeled projects and the other five semi-automated labeled projects. We did address in \S4.6 \citeresp{1h-1}. Moreover, we added an extra column in \tbl{data}c as the reviewed commits percentage for each project in order to retrieve 95\% of the bug-fixing commits, where the median is 22\% \citeresp{1h-2}. 

\review{\textbf{R1-i:} 3. Evaluation does not include the state-of-the-art. \\
The authors first proposed to leverage EMBLEM to identify which commit is bug-fixing. In the evaluations, the authors compared with a keyword-based approach. However, there are many approaches have been proposed to identify bug-fixing commits automatically, such as Relink \cite{Wu11_relink} and \cite{Tian12_linux}. Especially, in the work proposed by Tian et al. \cite{Tian12_linux}, they also compared with the keyword-based approach, which has already demonstrated an average improvement from 22.05\% to 50.07\%. Therefore, such important related works should be selected as baselines for comparison.}

We really appreciate these pointers into the literature. We carefully read the Relink \cite{Wu11_relink} and Lo et al. \cite{Tian12_linux} papers and we agree that there is an interesting connection from our work to that work which would be important to mention.

We would not say that Relink and Lo et al. are  alternative to the methods of this paper. In fact, we would say that our work is a \textit{preamble} to their work \citeresp{1i}:

\begin{quote}
 ``(Relink and Lo  et al.) assume the existence of some pre-labeled examples. For example, suppose we wish to certify the effectiveness of (say) the Lo et al. method. Such a certification would require a library of ground truth examples that some process has certified to have accurate labels. This paper discusses cost-effective methods for generating such a library of ground truth examples.''
\end{quote}

 

% Also, in another way,  the goal of theis paper is to propose an efficient method that can incorporate human expertise for labeling in a new domain (i.e. computational science development). Both mentioned approaches of Relink and Linux bug-fixing patches identification require the existence of labeled data in order to execute which EMBLEM can be effective and helpful for. \citeresp{1h}

\review{\textbf{R1-j:} The authors should also compare with the-state-of-the-art approaches for predicting bug-inducing commits. For example, Yang et al., proposed to leverage deep learning techniques to predict which commit is buggy \cite{yang2015deep}.}

% however, the reviewers might argue that the result may change when using state-of-the-art Yang's DL method.

Again, this point is similar to previous point where we do need clarify how our work is different than others. 
\bi
\item
There are many ways to use the labels - once we have them. But almost without exception, prior work has assumed that the (a) the labels exist and (b) the labels are correct.
\item
Now if you challenge those assumptions, and if you want to check if the labels are right, then that is a very labor-intensive process.
\item
What we show here is that we can reduce that labeling effort  by around an order of magnitude, using active learning.
\ei
As to Yang et al. \cite{yang2015deep} being state of the art, 
we quite take your point that researchers need to constantly watch the literature looking for new and better ways to perform standard tasks. 
But in the case of ``what is best for defect prediction?'', it is not clear to us that Yang et al. are the definitive source. For
example, the FSE'18 reviewers  for our FFT paper\cite{di18_fft},
accepted our argument that, when comparing new defect predictors to old ones, the Ghotra ICSE'15 study (which currently has 183 citations~\cite{ghotra15}) is a reasonable place to go to find reference systems. There are several reasons why the Ghotra et al. sample might be preferred to that of Yang et al; e.g. Ghotra et al. studied 32 different classifiers while Yang et al. studied just three.
For those reasons, we benchmarked FFTs against the Ghotra sample and found that FFTs worked best.
 


\review{\textbf{R1-k:} Recent studies have pointed out that the SZZ algorithm is not accurate. For instance, Böhme et al. [1] found that, for nearly one third of their studied bugs, SZZ cannot identify any real bug-inducing commits via “blaming” the statements modified by the bug-fixing commits. Costa et al. [2] later proposed a framework to evaluate the results of SZZ. They found that for 46.0\% of their studied bugs, the bug-inducing commits identified by SZZ are years apart from one another while it is unlikely that code changes committed years apart will induce the same bug. Have the authors checked such bias in their evaluation?}

You made a good point: there is much recent work in SZZ and its variants. 
 Lo et al. \cite{lo19_mislabeled} reported that the effectiveness of mislabeling the data affect on average different of 1\%-5\%. The results are suggestive but not conclusive that while fine tuning SZZ is important, comparing their results to ours, there may be more benefit in improving the knowledge input to the process (via EMBLEM's extracting more info from humans) than making adjustments to the data pre-processing (by tinkering with SZZ).  

But more importantly, your comment   highlights a structural flaw in the prior draft: {\em we did not emphasize that this work was about
stage 4 labeling} (as opposed to the rest of the data mining pipeline shown in \fig{pipeline}). This current draft makes that point much more explicitly, \citeresp{1i}.


Now referring to \fig{pipeline}, we note that there are many stages to the data mining problem. We mapped our pipeline to imitate \fig{pipeline} in \S2.2, SZZ runs in phase 5 (feature engineering)
while this paper is about phase 4 (data labeling). And apart from data collection and data labeling, there are seven other essential parts to the data mining
problem. We raise this since no single paper can cover all parts of this pipeline. So no, we do not study variants to SZZ for the same reason we do not study model requirements or feature engineering or model training or model evaluation or model deployment of model monitoring (i.e. one paper cannot do everything).


Just to say one more thing about the relationship of this work to the SZZ research:  we note in section 4.4 of a recent TSE paper on SZZ~\cite{costa17szz} that their evaluation methods for their new SZZ variant included a manual step where software artifacts were inspected. For other researchers to check the veracity of that manual evaluation step, that manual analysis would have to be repeated. Such manual inspections of software artifacts  can be a time-consuming process. Tools like ours could certainly help the SZZ research to have better reproducability of their results.
 
 
 

\review{\textbf{R1-l:} Some other typos. There are many typos in this manuscript. Please carefully fix these writing issues. Some examples are listed as follows: \\
\begin{itemize}
    \item   Page 5 line 37: “since many of these projects a simple one-person prototypes”
    \item   Page 6 line 36: “oroject data was divided into”
    \item   Page 8 line 14: “It method is applied and …”
\end{itemize}}

Thank you for your comment. We have carefully proof-read the manuscript to get rid pf the typos and grammar mistakes. 

\par ~

\subsection*{Response to Reviewer \#2}

Please see the \revised{WORDS IN BLUE}, showing exactly where we have updated this draft.
Also, please see below for our responses to your specific comments.

\review{\textbf{R2-a:} The contribution of the paper. The paper in all contributes in proposing using active learning in labeling commits. I do see the contribution part at the end of intro. However, honestly, number 1, i.e., “we bring this idea to you”, is not a contribution, but rather the paper itself. Number 3 is a bit weak since some of the subjects in this paper is also in Java and trying software defect prediction on a domain of software is although indeed a contribution, but not significant. Otherwise one can just pick a new domain, try it out and claim contribution. I hope the authors can support their contribution more in the rebuttal and convince me the significance of it (not just emphasizing the ones in page 3).}

Thank you for your comment. We agreed that the prior draft did not present the contributions adequately and we have revised the list of the contribution to reflect and support the contributions of the work \citeresp{2a-1}. Moreover, we have updated with an extra section (i.e. \S2.1) to provide the bigger picture how our method can contribute to the general area of data sharing and research reproducibility in software engineering (particularly) and science (generally). \citeresp{2a-2} 

\review{\textbf{R2-b:} The need of the approach. This is another major concern of mine. This technique, although useful in cases, may not be needed at all in many cases. Using issue tracking system to link issue reports to the commits and use the data in the issue reports to label the commit is a very common practice in software prediction. I understand there are always projects that are without an issue tracker. This makes me remember once upon a time, people study how to combine changes in CVS into change sets. If you ask me are those techniques useful, of course. There are still projects on the planet using CVS. But the relevance is decreasing. \\
In fact, I checked some of the subjects that the authors study, some of them have issue ids right in their commit messages and some do have an issue tracker, that you can mine to link back to the commits. \\
Hence I would like to ask the authors how useful is their approach considering the fact that one may link issue tracker to the version control and label commits based on that. My suggested way may be study how often a project (say in Github) do not use internal issue tracker or an external one. Or even the ones that use, how often the commits cannot be linked to an issue to be labeled, in order to better motivate the work.}

Great suggestions, we have updated the manuscript with how we checked the issues
(see Table~\ref{tbl:gittracking}) and   found that only 9\% of the total bug-fixing commits can be linked back to the issues while 3\% of the total issues can be found mentioned through the bug-fixing commit logs. 


Also, for one clear statement on why our methods are needed, please see our notes
on {\bf RQ3} on page 1 and 2: there we showed one example were a task costing \$320K and 39,000 hours (without our tools) would cost around \$40K and 4,940 hours (with our tools) which is an order of magnitude improvement. 

It is not the goal of this paper to link the issues with the bug-fixing commits but it is indeed that our EMBLEM can help generate the necessary bug-fixing commits to associate with the issues where they do not exist such as this case. \citeresp{2b}

\review{\textbf{R2-c:} Unclearness of the bug prediction models. By reading through RQ2 to RQ4, I am a bit confused about whether each RQ is doing commit level or file level bug prediction. I assume RQ2 is commit level bug prediction. But the highlight box of RQ2 in top left of page 9, says, buggy code. Also, the first line of page 9, “such code” should be “such commit”, I assume. Then RQ3, in the question, you say “buggy code” but in the highlight box, you say, “buggy commits”. Now I am completely confused. Or do you mean the same thing? Now in RQ4, the authors say, for RQ1 and 2, the target is for prediction task and for RQ3 it’s for analytic task. Does it mean that RQ1 and 2 are for commit-level and RQ3 if for file level? But now, is RQ4 commit level or file level? I would suggest the authors clarify this up and clearly lay this out in the paper ahead of time to avoid confusion.}

Good point, we are doing commit-level prediction for all the RQs. Therefore, all the unclears for ``code'' should be revised as commits appropriately. 

\review{\textbf{R2-d:} If there are file-level prediction, are the authors doing post release bug? If so, how is the post release determined? If the authors doing the commit-level prediction, did the authors pre-check the data generated by szz to avoid clear mistakes from szz and how do you control it? For example, sometimes, the szz would say a large number of commits are bug inducing to one bug.}

Good point, we are doing commit-level prediction where we focusing on the improvement of the labeling stage and seeing if that also benefiting the prediction stage. This point is answered extensively above in R1-k. Specifically referring to \fig{pipeline}, we note that there are many stages to the data mining problem. We mapped our pipeline to imitate \fig{pipeline} in \S2.2, SZZ runs in phase 5 (feature engineering)
while this paper is about phase 4 (data labeling). And apart from data collection and data labeling, there are seven other essential parts to the data mining
problem. We raise this since no single paper can cover all parts of this pipeline. So no, we do not study variants to SZZ for the same reason we do not study model requirements or feature engineering or model training or model evaluation or model deployment of model monitoring (i.e. one paper cannot do everything). 

Moreover, Lo et al. \cite{lo19_mislabeled} results showcased the impact of mislabeling is on average of 1-5\% difference. It is suggestive that where we acknowledge that while fine tuning SZZ is important, there may be more benefit in improving the knowledge input to the process (via EMBLEM's extracting more info from humans) than making adjustments to the data pre-processing (by tinkering with SZZ).


\review{\textbf{R2-f:} The title of the paper misses the important context of the paper, i.e., bug prediction. The authors should clear that up in the title. In addition, F3T, only the first F is about the labeling. The rest is not about the enhanced labeling. I wouldn’t put F3T in the title.}

Good point, we have updated the title to address this.  

\review{\textbf{R2-e:} In the paper, the authors use “buggy” or “not buggy” to describe the commits. I think it’s misleading. Maybe consider use “bug fixing” or “none bug fixing”. Also in the fist line of the conclusion, the authors should also mean “bug fixing” or “none bug fixing”. “Worrying” or not is an internal state in the active learning.}

Good point, we have updated to ``bug-fixing'' and ``none bug fixing''.

\review{\textbf{R2-g:} Table 10, the p20 part, first line, none of them wins?}

Yes, which means that the learners performed similarly. 

\review{\textbf{R2-h:} Personally I don’t see the value of section 2.3. I understand the authors may have their own concerns, but I personally would save that space to provide more details about the RQs.}

Thank you for your suggestions, we have updated the manuscript to include more details regarding the methods, motivations and the RQs of the papers. \S2.3 is also updated to \S2.2 which we think that it is important to elaborate on many software analytic tasks that our tool EMBLEM can be generalized to.   

\review{\textbf{R2-j:} Some typos, grammar issues, bad wordings: Page 1: abstract: humans the apply Abstract: “very effective” “very” is a vague word Page 2, RQ3 maybe What --$>$ Which? RQ4, which identification and prediction system performs the best for … Page 5, right column first line, than --$>$ then Page 8, bottom left, “RQ2,RQ3” --$>$ missing a white space before “RQ3” }

Thanks for your comment, we have updated the manuscript to accommodate these changes. 

\subsection*{Response to Reviewer \#3}

Please see the \revised{WORDS IN BLUE}, showing exactly where we have updated this draft.
Also, please see below for our responses to your specific questions.

\review{\textbf{3-a:} While the combination of previously established techniques is a strength of this paper on one hand, it also raises concerns about the size of the contribution of this work. Indeed, the most intriguing contribution of this work is the manual labeling of commit messages from a domain which is often overlooked in Software Engineering research, but I wonder if this is sufficient for a TSE publication. For a journal paper, I would expect a more detailed investigation of why EMBLEM and FFT work better than the baseline techniques in this scenario. What do they learn that other learners did not pick up on, for example?}

Please note that in response to your comments, we have significantly reorganized the  paper to better introduce and motivate and clarify this whole idea. In particular, this draft is far clearer on:
\bi
\item Why this work is needed: see the discussion around \tbl{gittracking};
\item What is the focus of this work: improving labeling quality through the EMBLEM method while FFTs is just an internal detail;
\item What are the contributions: in the draft, we distinguish our contributions in into the  bigger picture  (see \S2.1) and other parts of the data mining process specifically (see \S2.2);
\item What are the differences between EMBLEM and state-of-the-art ones: technical differences between the previous techniques and our EMBLEM (stopping mechanism and more informed learning method, see \S3.2) \citeresp{3a}.
\ei

As you quite rightly  point out, the previous description of this worked confused the core message with
some of the less-important implementation details.

Accordingly, we now focus here on our main message (the labeling) rather than certain less-important details (the learning method). We say FFTs are less important since, since in \tbl{rq2aaa}, we  compare the effects of using or not using FFTs in conjunction with the usage EMBLEM. The result there is very clear, if we use FFTs with EMBLEM, that wins over just using FFTs 
(without EMBLEM) in  7/9 cases in computational science projects  
(for both $P_{opt}20$ and G-score). Therefore, we say that the real message of this paper is EMBLEM and not FFTs.  

 
\review{\textbf{3-b:} The title of the paper refers to labeling of issue reports, yet the paper appears to be about commit message labeling. Should the title be adjusted?}

Good point, we have adjusted the title to fit the context of the revised manuscript (labeling commits). 

\review{\textbf{3-c:} I found the terminology of ``worrying'' vs. ``not-worrying'' confusing. Why is a commit message which contains the words ``fix'', ``better'', or ``test'' (for example) worrying? If anything, I would argue that these indicate commits which would make me worry less.}

Good point, we have updated the terminology ``worrying'' to ``bug fixing'' as it was supposed to identify bug-fixing commits through reading commit message.

\review{\textbf{3-d:} Related to the previous point, the authors claim that Table 1 (the worrying keywords) are taken from reference 33. This does not appear to be correct -- although the Commit Guru paper claims the same. Would the authors be able to point out exactly where in reference 33 these keywords are to be found? A quick search didn't come up with anything, but I may have missed it. I suspect that the keywords were introduced in the Commit Guru paper instead of the Hindle 2008 work.}

Thanks for noticing that, we took the keywords from Commit Guru paper \cite{commitguru} which cited and said to leverage the Hindle 2008 work \cite{hindle08_largecommits}. I have updated the reference to only Commit Guru paper.  

\review{\textbf{3-e:} While the focus on computational science software is a nice feature of this paper, it does beg the question whether the same improvements would be achieved on the projects that have been studied in related work. I would suggest that the authors report the results of their approach on at least one of the projects that were used by related work. This would also provide some data on the extent to which the domain affects the performance of different approaches.}

You ask for ``at least one more data set''. That is such a good idea
that  we did two.
We have inspected this also on the two standard SE projects of Eclipse JDT and Eclipse Platform (i.e. sample of standard SE projects that was suggested in several commit-level defect prediction \cite{kamei12_jit, yang2015deep}) where we did not find the same improvements achieved for those from computational science projects. We recorded our findings in RQ3 and provided remarks on how the domain affects the performance of the different approaches.  \citeresp{3e} 



\review{\textbf{3-f:}  For the manual labeling, the authors report "very low" observed disagreement and that it was under 15\%. Please provide the exact numbers, ideally along with a representative example of a disagreement.}

Good point, the exact number is 14.6\% and we have provided some of the examples of disagreement for manual labeling as well. We observed that the human labelers have disagreements where (1) attempts to fix might not guarantee an actual bug-fixing activity (e.g. RMG-PY, HOOMD, and PCMSOLVER examples) and (2) ``fixes'' that might not be quantified as true bug-fixing activities (e.g. AMBER and XENON). \citeresp{3f}

\review{\textbf{3-g:} For the labels generated by EMBLEM, the recall on the PCMSOLVER data set is quite a bit lower than for the other four data sets (Table 6). It would be good to provide an explanation for this difference.}

It is a sample of 100 commits over the whole project and we suspected that the lower recall was affected by the disagreements between the manual labelers and EMBLEM concentrated there more. We also have provided examples and observations of these disagreements in \S4.6 \citeresp{3f}.

\review{\textbf{3-g:} I would strongly encourage the authors to proofread papers before submission -- it is quite irritating to review a manuscript which was prepared without care. A few examples mostly from the first page, but note that this list is nowhere near complete:
\\ Humans the apply --$>$ Humans then apply
\\ commits that they guess is --$>$ are
\\ bugs labels --$>$ bug labels
\\ commits that indicates --$>$ indicate
\\ squares of Figure 1 shows --$>$ show
\\ a semi-automatic methods --$>$ method
\\ oroject --$>$ project
\\ ahve --$>$ have
}

Thank  your  for  the  comments.  We  have  proof-read  it  again to resolve the readability concern.

==> older/datasets.tex <==
\begin{table}[!t]
\begin{center}
\caption{Dataset statistics. Data was mined and curated from each own open project's github repository.}
\label{tb:dataset}
\begin{tabular}{c@{~}|r@{~}|r@{~}|r@{~}}
\begin{tabular}[c]{@{}c@{}} \textbf{Dataset} \end{tabular} &  \begin{tabular}[c]{@{}c@{}} \textbf{No. of Commits}\end{tabular} & \textbf{No. of Releases} & \begin{tabular}[c]{@{}c@{}} \textbf{Severe \%}\end{tabular} \\ \hline
pcmsolver & 1655 & 2  & 11  \\ 
xenon & 1804 & 7  & 19  \\ 
mdanalysis & 2733 & 8  & 20  \\  
hoomd & 3904 & 8  & 26 \\ 
abinit & 3911 & 9 & 32  \\  
amber & 4243 & 4  & 23 \\ 
rmg-py & 4472 & 7 & 14 \\ 
lammps & 5587 & 7 & 24 \\ 
libmesh & 7801 & 10 & 34 \\ 

\end{tabular}
\end{center} 
\vspace{-0.5cm}
\end{table}

==> older/temp.tex <==

% Data acquisition comes prediction.  State-of-the-art data mining methods for software analytics include Synthetic Minority Oversampling Techniques (SMOTE) to handle class imbalance \cite{agrawal2018better, kamei12_jit} in combination with standard miners (Random Forest (RF), Logistic Regression (LR), and Support Vector Machine (SVM)). However, Chen et al. \cite{di18_fft} recommended Fast-Frugal Trees as the prediction model where it demonstrated that the model have dominated other standard methods for defect prediction and close issues prediction. Therefore, our recommended system to explore and improve the state-of-the-art risky software prediction of $F^3T$ as the combination of FASTREAD labeling method and FFTs predicting model will be validated with the comparisons against other standard data mining methods and answering the following research questions:

%         \textbf{RQ1: { How close are FASTREAD and Keyword Labeling to Human Labeling?}}
 
% Software maintenance is a continuing process, and software developers have the domain expertise in understanding the commit logs. 25,000+ commits are crossed labeled by SE Ph.D. students from 4 projects. With the initial assumption that software maintenance requires the expert's understanding, these human-labeled commit logs data from those four initial sampled repositories serves as the ground truth to compare the effectiveness of automatic Keywords versus FASTREAD tagging. FASTREAD statistically significant won across four cases with our three evaluation metrics of precision, recall, and false-alarms (up to 38\% precision, 31\% recall and 111\% false-alarm).
 
 %Four popular repositories that satisfy our sanity checks were picked at random, and their commit logs were sampled to be labeled for bug-fixing commits by a human. 

% \begin{RQ}{}
% \vspace{-10pt}

% FASTREAD as the method for bug-fixing commits augmentation is better than current automatic keyword tagging.
% \end{RQ}
 
 
%          \textbf{RQ2: { How are risky software commit prediction based on FASTREAD labeled data perform against state-of-the-art method (Keyword) labeled data?}}
  
% %From the bug-fixing commits, we can track back to find bug-inducing commits that introducing defects to the software. Each of these commits will be analyzed, and recommended metrics are extracted to describe how risky each commit is. 

% The right green flow in Figure \ref{fig:system} demonstrated our approach to improve the correctness of finding the bug-fixing commits. When the right bug-inducing commits are linked and analyzed to extract relevant values of metrics, a more robust model to predict future risky software commits is built. FFTs is validated as our chosen data miner when FFTs dominated the three standard methods (SMOTE+RF, SMOTE+LR, and SMOTE+SVM) in our experiment described in section 4 (RQ2). By winning 7 (78\%) for G-score and 6 (67\%) for $P_{\mathit{opt}}$ out of 9 projects, FFTs model built on FASTREAD labeled data outperform FFTs model built on Keyword labeled data. 
 

% \begin{RQ}{}
% \vspace{-10pt}
% FASTREAD labeled data are more fit and higher quality for risky software commit prediction. Automatic Keywords labeling method for defective software commit is deprecated for future defect prediction work.  
% \end{RQ}
  

%         \textbf{RQ3: {How state-of-the-art risky software commit identification and prediction system, Commit.Guru, comparing to our recommended $F^3T$ system in predicting risky software commit?}}
 
% %Data quality also comes from the proportion of the labels within the dataset. Agrawal et al. \cite{agrawal2018better} has found that imbalance class problem is apparent within defect prediction research. Although our study is not defect prediction, it does inherit a lot of defect prediction problem's nature where most of the commits are not bug-inducing commits. Risky software commit prediction also exhibit an imbalance class problem. Outside of data quality, data miner should be chosen carefully to leverage the nature of the problem and the dataset itself. 

% Current state-of-the-art risky software commit identification and prediction system is Commit.Guru (Keyword + Logistic Regression) that illustrated in the left blue flow in Figure \ref{fig:system}. However, FASTREAD is proven to improve the dependent features quality, or the correctness of risky software commit identification, the target for prediction task (from RQ1 and RQ2) while FFT has proven to be a robust data miner for software analytics task. Our proposed system of $F^3T$ (FASTREAD+FFTs) dominated on G-scores with statistically significants win on all 9 projects and improvement  of the absolute delta up to 48\%. For $P_{\mathit{opt}}$,  $F^3T$ won 7 out of 9 projects with the absolute delta up to 26\%. 

  
% \begin{RQ}{}
% \vspace{-10pt}
% $F^3T$ outperformed state-of-the-art risky software commit identification and prediction system, Commit.Guru. $F^3T$ is recommended as a new baseline for future research work.
% \end{RQ}

% %          extbf{RQ4: { How the FFT model comparing to state-of-the-art methods in predicting risky software commit?}}
 
% %  Modern state-of-the-art methods do include more than just Logistic Regression such as Random Forest (RF) and Support Vector Machine (SVM) for more complex problems in combination with Synthetic Minority Oversampling Technique (SMOTE) to handle class imbalance problem. It is essential to validate our data miner of choice FFT by comparing it against state-of-the-art data miners. With seven wins, one loss, and one tie, FFT model outperformed state of the art data miner in risky software commit prediction.  

 
% % \begin{RQ}{}
% % \vspace{-10pt}
% % FFT model outperformed state-of-the-art risky software commit prediction and is recommended as a new baseline for future work in risky software commit prediction.
% % \end{RQ}


% % \subsection{Experimental Rig}

% % \noindent         \textbf{Step 1: Bug-fixing commits augmentation.} For the initial four main projects (ABINIT, libMesh, MDANALYSIS, and LAMMPS), the commit logs are cross-labeled by two graduate students in SE research. Total of 9 projects are augmented by both automatic Keyword tagging method and FASTREAD method. 

% % \noindent         \textbf{Step 2: Bug-inducing change identification.} To link bug-fixing commits and their bug-inducing commits (e.g. crash, bug, issues), the well-known SZZ algorithm that is designed by Sliwerski and improved by Kim et al. is employed \cite{Sliwerski05changes, Kim08changes}.  

% % \noindent         \textbf{Step 3: Metrics Collection.} The recommended 14 metrics to study defect-prone commits by Kamei et al. \cite{kamei12_jit} from Table \ref{tbl:metrics} for each project are recorded by depriving from the source code control system (e.g., Git).  

% % \noindent         \textbf{Step 4: Data Preprocessing.} Current software analytics work include data transformation and prediction. Before experimenting with standard data miners, the data will be ``SMOTEd'' to handle class-imbalance, which was not considered in Commit.Guru. 

% % \noindent         \textbf{Step 5: Data Mining.} We adopted the incremental learning approach for this study where release $i$ of project $j$ is trained and test on release $i+1$. 
% % For the initial four projects (ABINIT, LIBMESH, LAMMPS, and MDANALYSIS), $j_i[keyword]$ and $j_i[FASTREAD]$ will be trained and test on $j_{i+1}[human]$. From that result, we are confident to scale up without human labels as ground-truth bug-fixing labels. 
% % Therefore, for the rest five projects, $j_i[keyword]$ and $j_i[FASTREAD]$ \hspace{0.05cm} will be trained to test on \hspace{0.05cm} $j_{i+1}[keyword]$ \hspace{0.05cm} and $j_{i+1}[FASTREAD]$ respectively. 
% % For this study, we comparing Fast-Frugal Trees against Support Vector Machine, Random Forest, and Logistic Regression (state-of-the-art data miner). The process is repeated 20 times to mitigate biases.  


% % \subsection{Systematic Commit Logs Labeling}

% % FASTREAD algorithm \cite{Yu2018} augmented bug-fixing commits by:
% % \begin{enumerate}
% %     \item Input thousands of commits per project.
% %     \item Initial random reasoning phase: humans to skim through the commits messages manually until they have found $|L_R| \geq 1$ bug-fixing commit (along with $|L_I|$ non bug-fixing ones). Dozens of both categories of commits should be found before next step.
% %     \item Reflective reasoning phase (Line 6-7 \cite{Yu2018})
% %     \bi
% %     \item The Support Vector Machine (SVM) model is trained on the $L$ examples. When $|L_R \leq 30|$, aggressive undersampling  are employed to reject all the non bug-fixing commits. 
% %     \item Uncertainty sampling of commits with highest uncertainty of category when $|L_R \leq 30|$ (line 25) and certainty sampling of commits with highest probability to be bug-fixing when $|L_R \geq 30|$ (line 27).   
% %     \item Iterate the reflective reasoning phase until more than 95\% of the bug-fixing commits have been found ($|L_R| \geq 0.95|R|$).
% %     \ei
% % \end{enumerate}




% %\subsection{Statistical Testing}

% %We compared our results of tuned miners per release version using statistical significance test and an effect size test by Scott-Knott procedure \cite{mittas2013ranking, ghotra15}. Significance test detects if two populations differ merely by random noises \cite{ghotra15}. Effect sizes checks whether two populations differ by more than just a trivial amount, where $\mathit{A12}$ effect size test was used \cite{arcuri2011practical}. Our stats test are statistically significant with 95\% confidence and not a ``small'' effect ($\mathit{A12} \ge 0.6$).



% \section{Results}



%         \textbf{RQ1: { How close are FASTREAD and Keyword Labeling to Human Labeling?}}
 
% Software maintenance is a continuing process and software developers have the domain expertise in understanding the commit logs. Four popular repositories (ABINIT, LAMMPS, LIBMESH, and MDANALYSIS) that satisfies our sanity checks were picked at random and their commit logs were sampled to be labeled for bug-fixing commits by human. With the initial assumption that software maintenance requires the expert's understanding, these human labeled commit logs data from those four repositories serves as the ground truth to compare the effectiveness of automatic keywords tagging versus FASTREAD tagging. Table \ref{tab:rq1} is very clear and we can conclude that FASTREAD won significantly on all three evaluations metrics (precision: 8\%-21\%, recall: 11\%-23\%, and especially in false-alarm 8\%-38\%). Interestingly, between false-alarm and recall relationship, if one metric is optimized, the other usually declined. However, from our initial results on just labeling comparing with manual human ground truths labels, FASTREAD labels to identify software bug-fixing commits are very close to how a developers would label them. 

% \begin{RQ}{}
% \vspace{-10pt}
% FASTREAD as the method for bug-fixing commits augmentation is better than current automatic keyword tagging.
% \end{RQ}





%         \textbf{RQ2: { How are risky software commit prediction based on FASTREAD labeled data perform against state-of-the-art method (Keyword) labeled data?}}
 


% % \begin{table}[!t]
% % \footnotesize
% % \begin{center}
% % \begin{tabular}{c@{~}|r@{~}|r@{~}|r@{~}|r@{~}}
% % \multicolumn{1}{c|}{} & \multicolumn{4}{c}{        \textbf{\% $P_{\mathit{opt}}$ Wins}} \\
% % \cline{2-5}
% % \begin{tabular}[c]{@{}c@{}}         \textbf{Dataset} \end{tabular} & \begin{tabular}[c]{@{}c@{}}            \textbf{SMOTE+RF}\end{tabular} &         \textbf{SMOTE+SVM} & \begin{tabular}[c]{@{}c@{}}         \textbf{SMOTE+LR}\end{tabular} &         \textbf{FFT} \\ \hline
% % PCMSOLVER & 0 & 0 & 0 & 0  \\ 

% % LAMMPS & 37 & 0 & 0 & 12  \\  

% % HOOMD & 0 & 0 & 0 & 20  \\  
% % MDANALYSIS & 28 & 0 & 0 & 28\\ 
% % XENON  & 16 & 0 & 0 & 33\\ 
% % ABINIT & 0 & 0 & 0 & 37 \\ 
% % LIBMESH & 12 & 0 & 0 & 50\\ 
% % AMBER & 0 & 33 & 0 & 66  \\ 
% % RMG-PY & 0 & 0 & 0 & 80\\ 

% % \end{tabular}
% % \end{center} 
% % \vspace{-10pt}
% % \end{table}

  
% From the bug-fixing commits, we can track back to find bug-inducing commits that introducing defects to the software. Each of these commits will be analyzed and recommended metrics are extracted to describe how risky each commit is. Finding the right bug-inducing commits will help to link to the right bug-inducing commits with appropriate values of metrics to build a strong model to predict future risky software commits. Our recommended data mining method is FFT with no preprocessing. Essentially, we wanted to compare $F^3T$ (FASTREAD+FFT) and Keyword+FFT.
 
 
 
%  In order to validate our chosen data miner, FFTs, we evaluated the performance of it by building FFTs on FASTREAD labeled data against standard methods (SMOTE+SVM, SMOTE+RF, and SMOTE+LR). Table \ref{tb:rq4} provides the statistical testing results for G-score (top) and $P_{\mathit{opt}}$ (bottom) performances. For G-score, FFT dominated in most of the releases, 7 wins out of 9 projects while performing similarly in 1 case (in AMBER) and losing to SMOTE+LR in 1 case (in PCMSOLVER) when 6 wins have 50\% and above win. For $P_{\mathit{opt}}$, FFT performance also have the most win percentages in most of the releases, 6 wins out of 9 projects while performing similarly to other data mining methods in 2 cases (PCMSOLVER and MDANALYSIS) and losing to SMOTE+RF in 1 case (in LAMMPS).  Figure \ref{fig:rq4} provides the median absolute delta performance insight from each project numerically between FFTs and state-of-the-art data mining methods (SMOTE+RF, SMOTE+SVM, and SMOTE+LR). We can see: (1) RF is widely adopted in defect prediction task but surprisingly doing worst in G-score (when comparing with FFTs for the median delta difference across all releases); (2) The good performance of SMOTE+LR when comparing to SMOTE+RF and SMOTE+SVM in G-score is evidental to why even though LR is deprecated in defect prediction task, it is widely adopted in JIT defect prediction \cite{commitguru}; (3) FFTs model outperformed standard data mining methods is validated as our chosen data miner. 


% % \begin{figure}[!t]
% % \includegraphics[width=\linewidth]{rq4_2.png}
% % \vspace{-25pt}
% % \end{figure}
 
% \begin{table}
% \small
% \begin{center}
% \caption{RQ2 Statistical Result - G-score (left) and $P_{\mathit{opt}}$ (right) percentage performance comparison of statistically significant wins across all the releases per project between FASTRERAD+FFT($F^3T$) versus Keyword+FFT(K+FFT)}
% \label{tb:rq2}
% \resizebox{\linewidth}{!}{
%  \begin{minipage}{0.55\linewidth}
% \begin{tabular}{c@{~}|r@{~}|r@{~}}
% \multicolumn{1}{c|}{} & \multicolumn{2}{c}{        \textbf{\% G-score Wins}} \\
% \cline{2-3}
% \begin{tabular}[c]{@{}c@{}}         \textbf{Dataset} \end{tabular} & \begin{tabular}[c]{@{}c@{}}         \textbf{K+FFT}\end{tabular} &         \textbf{$F^3T$}\\ \hline
% PCMSOLVER & 100 & 0  \\ 
% AMBER & 67 & 33  \\ 
% HOOMD & 40 & 60 \\ 
% RMG-PY  & 40 & 60 \\ 
%         \textbf{ABINIT} &         \textbf{25} &         \textbf{62} \\ 
%         \textbf{LIBMESH} &         \textbf{28} &         \textbf{72}  \\  
%         \textbf{MDANALYSIS} &         \textbf{28} &         \textbf{72} \\ 
%         \textbf{LAMMPS} &         \textbf{25} &         \textbf{75} \\
% XENON & 16 & 83  \\  
% \end{tabular}  %
% \end{minipage} \
% \begin{minipage}{0.55\linewidth}
% \begin{tabular}{c@{~}|r@{~}|r@{~}}
% \multicolumn{1}{c|}{} & \multicolumn{2}{c}{        \textbf{\% $P_{\mathit{opt}}$ Wins}} \\
% \cline{2-3}
% \begin{tabular}[c]{@{}c@{}} 
%         \textbf{Dataset} \end{tabular} & \begin{tabular}[c]{@{}c@{}}         \textbf{K+FFT}\end{tabular} &         \textbf{$F^3T$}\\ \hline
% AMBER & 67 & 33  \\
% HOOMD & 60 & 40 \\ 
% XENON & 50 & 50  \\  
%         \textbf{LAMMPS} &         \textbf{37} &         \textbf{50} \\
%         \textbf{ABINIT} &         \textbf{37} &         \textbf{50} \\ 
%         \textbf{MDANALYSIS} &         \textbf{42} &         \textbf{57} \\ 
% RMG-PY & 20 & 80 \\ 
%         \textbf{LIBMESH} &         \textbf{14} &         \textbf{86}  \\  
% PCMSOLVER & 0 & 100  \\ 
% \end{tabular}
% \end{minipage}}
% \end{center} 
% \vspace{-10pt}
% \end{table}




 
%  Figure \ref{fig:rq2} provides the median performance insight from each project for each release numerically between $F^3T$ and Keyword+FFT for G-score (top chart) and $P_{\mathit{opt}}$ (bottom chart). The blue diamond represents $F^3T$ while the black circle represents Keyword+FFT A lot of the differences between the two methods are easy to spot (i.e. performance on $P_{\mathit{opt}}$ chart for RMG-PY), but some are not (i.e. performance on G-score chart for AMBER). In order to confirm our hypothesis,
%  the percentage of statistically significant winning or ranking higher across all the releases in each project are recorded in Table \ref{tb:rq2}. Specifically, for LAMMPS, there are 9 releases, so the performance metrics are collected 8 times incrementally and FFT model built on FASTREAD generated data won 6/8 for G-score and 4/8 for $P_{\mathit{opt}}$  so $F^3T$ won 75\% time for G-score and 50\% for $P_{\mathit{opt}}$ in LAMMPS. The higher number between the twos is the better combination method. Four initial datasets that got human ground truth labels are expressed in bold entries. We observe that four out four, $F^3T$ statistically overwhelm Keyword+FFT using the "Human labeled" ground truths.  
 






% Manual human labeled ground truths are important for the data mining process but expensive to get and hard to repeat. Original four initial datasets provide plentiful evidence for us to have confidence in FASTREAD generated risky software prediction data. In order to confirm that hypothesis, the experiment is repeated without human ground truth labels by testing only on the next release that was generated from the same labeling method(i.e., a learner that was trained on ABINIT Keyword release 1 will predict on ABINIT Keyword release 2 and a learner that was trained on ABINIT FASTREAD release 1 will be tested on ABINIT FASTREAD release 2). It is similar to previous studies that solely using automating Keyword  \cite{nayrolles18_clever, commitguru}. 


% With 7 and 6 wins out of 9 projects for G-score and $P_{\mathit{opt}}$ respectively, FFTs model built on FASTREAD generated data outperformed FFTs model built on Keyword generated data. Hence, 

% \begin{RQ}{}
% \vspace{-10pt}
% FASTREAD labeled data are more fit and higher quality for risky software commit prediction. Automatic Keywords labeling method for defective software commit is deprecated for future defect prediction work.  
% \end{RQ}

% \begin{table}
% \small
% \begin{center}
% \caption{RQ3 Statistical Result - G-score (left) and $P_{\mathit{opt}}$ (right) percentage performance comparison of statistically significant wins across all the releases per project between $F^3T$ versus Commit.Guru}
% \label{tb:rq3}
% \resizebox{\linewidth}{!}{
%  \begin{minipage}{0.52\linewidth}
% \begin{tabular}{c@{~}|r@{~}|r@{~}}
% \multicolumn{1}{c|}{} & \multicolumn{2}{c}{        \textbf{\% G-score Wins}} \\
% \cline{2-3}
% \begin{tabular}[c]{@{}c@{}} \end{tabular} & 
% \begin{tabular}[c]{@{}c@{}}
%         \textbf{Commit}\end{tabular} & \\
%         \textbf{Dataset}  &          \textbf{Guru} &         \textbf{$F^3T$}\\\hline
% XENON & 16 & 66  \\ 
% LAMMPS & 0 & 75 \\ 
% HOOMD & 20 & 80 \\ 
% ABINIT  & 0 & 87 \\ 
% AMBER & 0 & 100 \\ 
% RMG-PY & 0 & 100 \\ 
% LIBMESH & 0 & 100 \\ 
% PCMSOLVER & 0 & 100 \\  
% MDANALYSIS & 0 & 100  \\ 
% \end{tabular} \qquad
% \end{minipage}
% \begin{minipage}{0.5\linewidth}
% \begin{tabular}{c@{~}|r@{~}|r@{~}}
% \multicolumn{1}{c|}{} & \multicolumn{2}{c}{        \textbf{\% $P_{\mathit{opt}}$ Wins}} \\
% \cline{2-3}
% \begin{tabular}[c]{@{}c@{}} \end{tabular} & \begin{tabular}[c]{@{}c@{}}         \textbf{Commit}\end{tabular} & \\
%         \textbf{Dataset}  &          \textbf{Guru} &         \textbf{$F^3T$}\\\hline
% PCMSOLVER & 100 & 0  \\ 
% AMBER & 67 & 33  \\ 
% HOOMD & 40 & 60 \\ 
% RMG-PY  & 40 & 60 \\ 
% ABINIT & 25 & 62 \\ 
% LIBMESH & 28 & 72  \\  
% MDANALYSIS & 28 & 72 \\ 
% LAMMPS & 25 & 75 \\
% XENON & 16 & 83  \\  

% \end{tabular}
% \end{minipage}}

% \end{center} 
% \vspace{-15pt}
% \end{table}

% % \begin{figure*}[!t]
% % \caption{RQ3 Numerical Results - Median G-score (top chart) and $P_{\mathit{opt}}$ (bottom chart) performance of comparing the performance between $F^3T$ and Commit.Guru for each release per project.}
% % \includegraphics[width=\linewidth, height=1.8in]{rq3_1.png}
% % \label{fig:rq3}
% % \vspace{-20pt}
% % \end{figure*}
% % \begin{figure*}[!t]
% % \includegraphics[width=\linewidth, height=1.8in]{rq3_2.png}
% % \vspace{-20pt}
% % \end{figure*}

% \textbf{RQ3: {How state-of-the-art risky software commit identification and prediction system, Commit.Guru, comparing to our recommended $F^3T$ system in predicting risky software commit?}}
 
% Beside dependent ground truth labels, data quality also comes from the proportion of the labels within the dataset. Agrawal et al. \cite{agrawal2018better} has found that the imbalance class problem is apparent within defect prediction research. Although, our study is not defect prediction, it does inherit a lot of defect prediction problem's nature where most of the commits are not bug-inducing commits as shown in Table \ref{tbl:dataset} where the median of defective commit is 23\%. Therefore, risky software commit also exhibit imbalance class problem. Outside of data quality, data miner should be chosen carefully to leverage the nature of the problem and the dataset itself. FASTREAD improves the dependent features quality or the correctness of risky software commit identification, target for prediction task (from RQ1 and RQ2) while FFTs model has proven to be a strong data miner for software analytics task. Our recommended $F^3T$ method is chosen for this paper to compare against state-of-the-art risky software prediction method, Commit.Guru's Keyword+LR. 

% From the Figure \ref{fig:rq3}, the green triangles and red squares represent $F^3T$'s performance and Commit.Guru's performance for G-score (top chart) and $P_{\mathit{opt}}$ (bottom chart). $F^3T$ clearly outperformed Keyword+LR on all 9 projects for G-score where $F^3T$ won 100\% of the time in 5 projects for all the releases within that same project (recorded Table \ref{tb:rq3}). For $P_{\mathit{opt}}$, $F^3T$ won 7 out of 9 projects with statistically significant differences in the right of Table \ref{tb:rq3}. With the majority won on both measures, we can conclude: 


% \begin{RQ}{}
% \vspace{-10pt}
% $F^3T$ outperformed state-of-the-art risky software commit identification and prediction system, Commit.Guru. $F^3T$ is recommended as a new baseline for future research work.
% \end{RQ}




% %         extbf{RQ4: { How FFT model comparing to state-of-the-art data mining methods in predicting risky software commit?}}
 
% % Modern state-of-the-art methods does include more than just Logistic Regression such as Random Forest and Support Vector Machine for more complex problems in the combination with Synthetic Minority Oversampling Technique (SMOTE) to handle class imbalance problem. It is essential to validate our data miner of choice (i.e. FFTs), by comparing against state-of-the-art data mining methods in SE research. 

% % \begin{figure}[!t]
% % \vspace{-10pt}
% % \caption{RQ4 Numerical Difference Result - Absolute median delta of G-score (top chart) and $P_{\mathit{opt}}$ (bottom  chart) of comparing the performances between FFTs and state-of-the-art methods (SMOTE+SVM, SMOTE+RF, and SMOTE+LR)}
% % \includegraphics[width=\linewidth, height=1.8in]{rq4_1.png}
% % \label{fig:rq4}
% % \vspace{-25pt}
% % \end{figure}
% % \begin{figure}[!t]
% % \includegraphics[width=\linewidth, height=1.8in]{rq4_2.png}
% % \vspace{-25pt}
% % \end{figure}

% % The experiment and evaluation are similar to RQ2 and RQ3 but only training and testing on FASTREAD generated data. Table \ref{tb:rq4} provides the statistical testing results for G-score (top) and $P_{\mathit{opt}}$ (bottom) performances of comparing FFTs with SMOTE+RF, SMOTE+SVM, and SMOTE+LR. For G-score, FFT dominated in most of the releases, 7 wins out of 9 projects while performing similarly in 1 case (in AMBER) and losing to SMOTE+LR in 1 case (in PCMSOLVER) when 6 wins have 50\% and above win. For $P_{\mathit{opt}}$, FFT performance also have the most win percentages in most of the releases, 6 wins out of 9 projects while performing similarly to other data mining methods in 2 cases (PCMSOLVER and MDANALYSIS) and losing to SMOTE+RF in 1 case (in LAMMPS).  Figure \ref{fig:rq4} provides the median absolute delta performance insight from each project numerically between FFTs and state-of-the-art data mining methods (SMOTE+RF, SMOTE+SVM, and SMOTE+LR). We can see: (1) RF is widely adopted in defect prediction task but surprisingly doing worst in G-score (when comparing with FFTs for the median delta difference across all releases); (2) The good performance of SMOTE+LR when comparing to SMOTE+RF and SMOTE+SVM in G-score is evidental to why even though LR is deprecated in defect prediction task, it is  widely adopted in JIT defect prediction \cite{commitguru}. Finally, 


% % \begin{RQ}{}
% % \vspace{-10pt}
% % FFT model outperformed state-of-the-art risky software commit prediction and is recommended as a new baseline for future work in risky software commit prediction.
% % \end{RQ}


==> oometrics.tex <==

\begin{table*}[!t]
\footnotesize
\centering
\vspace{-0.35cm}
\caption{Object Oriented Measures used in our defect datasets }
\vspace{-5pt}
\label{tbl:oometrics}
\resizebox{\linewidth}{!}{
\begin{tabular}{l|l|l|p{12cm}|}
\hline
\rowcolor{gray!80}Metric & Name & Description \\\hline
\multirow{4}{*}{Diffusion} & NS & Number of modified subsystems & Changes modifying many subsystems are more likely to be defect-prone \\\hline{1-3}
& NS & Number of modified subsystems & Changes modifying many subsystems are more likely to be defect-prone \\\hline{1-3}
& NS & Number of modified subsystems & Changes modifying many subsystems are more likely to be defect-prone \\\hline{1-3}
& NS & Number of modified subsystems & Changes modifying many subsystems are more likely to be defect-prone \\\hline

\end{tabular}}
\vspace{-0.2cm}

\end{table*}

==> runtime.tex <==
\pdfoutput=1
\begin{table}[!t]

\caption{Runtime in seconds.}\label{fig:runtime}
\vspace{-5pt}

%~\\
%\setlength{\abovecaptionskip}{10pt plus 2pt minus 1pt}


\footnotesize
\begin{tabular}{r|cccc}

%   & ~ABE0 & ~ATLM & ~RD40 & ~RD160 & ~DE2 & ~DE8 \\ 
%\hline
%kemerer   & $<$1	 & $<$1	 & 3	& 13	& 4	& 10	\\
%albrecht   & $<$1	 & $<$1	 & 3	& 11	& 4	& 11	\\
%isbsg10   & $<$1	 & $<$1	 & 3	& 15	& 4	& 14	\\
%finnish   & $<$1	 & $<$1	 & 4	& 14	& 5	& 14	\\
%miyazaki   & $<$1	 & $<$1	 & 5	& 16	& 6	& 16	\\
%maxwell   & $<$1	 & $<$1	 & 12	& 52	& 18	& 53	\\
%desharnais   & $<$1	 & $<$1	 & 13	& 54	& 17	& 55	\\
%kitchenham   & $<$1	 & $<$1	 & 21	& 80	& 28	& 94	\\
%china   & $<$1	 & $<$1	 & 57	& 232	& 52	& 243	\\

 & ~CART & ~KNN & ~RF & ~SVM \\ 
\hline
Grid    &  4  &   5    & 9 & 6 \\ 
DE      & 4  &   5    & 8 & 6 \\  
Random  & 4  &   5    & 8 & 6 \\ 
Default & 1  &   1    & 2   & 1 \\  
SMAC    & 613     &   501    & 652 & 505  \\ 


\end{tabular}
\vspace{-17pt}
\label{tbl:runtimes}
\end{table}

